Volumetric Rendering with Baked Quadrature Fields

We propose a novel Neural Radiance Field (NeRF) representation for non-opaque scenes that enables fast inference by utilizing textured polygons. Despite the high-quality novel view rendering that NeRF provides, a critical limitation is that it relies on volume rendering that can be computationally expensive and does not utilize the advancements in modern graphics hardware. Many existing methods fall short when it comes to modelling volumetric effects as they rely purely on surface rendering. We thus propose to model the scene with polygons, which can then be used to obtain the quadrature points required to model volumetric effects, and also their opacity and colour from the texture. To obtain such polygonal mesh, we train a specialized field whose zero-crossings would correspond to the quadrature points when volume rendering, and perform marching cubes on this field. We then perform ray-tracing and utilize the ray-tracing shader to obtain the final colour image. Our method allows an easy integration with existing graphics frameworks allowing rendering speed of over 100 frames-per-second for a $1920\times1080$ image, while still being able to represent non-opaque objects.

==> Tables/fur-synthetic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|lll|lll}
\hline
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{Hairy monkey}} & \multicolumn{3}{c}{\textbf{Smokey monkey}} \\
 \cline{2-7}
                         & \textbf{PSNR}     & \textbf{LPIPS}     & \textbf{SSIM}      & \textbf{PSNR}      & \textbf{LPIPS}     & \textbf{SSIM}      \\

\hline
NGP + SG                     & 36.78    & 0.1585    & 0.9669    & 44.05     & 0.1432    & 0.9807    \\
\hline
NeuS~\cite{wang2021neus} & 22.81    & 0.1504    & 0.9069    & 23.34     & 0.1132    & 0.9148    \\
Ours                     & 34.76    & 0.1626    & 0.9565    & 35.86     & 0.1687    & 0.9546   \\
\hline
\end{tabular}%
}
\caption{\textbf{Evaluation on synthetic fur dataset.} We compare our approach with NeuS by surface rendering.}
\label{tab:fur-synthetic}
\end{table}

==> Tables/hardware.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{llll}
\toprule
                        & FPS @4096       & FPS @8192 \\
\hline
Macbook pro (M2)            &  15        &        8  \\
Desktop Nvidia-3090      &  20         &       9  \\
Desktop Nvidia A-6000     &  30          &        10 \\
% Mobile phone            &            &              &                      \\
\bottomrule
\end{tabular}
}
\caption{Evaluation of rendering speed is done with different texture sizes on the mic model from the synthetic dataset with $780k$ faces.
\label{tab:fps}
}
\end{table}

==> Tables/transparent.tex <==
\begin{table}[]

\begin{tabular}{llllll}
\toprule
            & PSNR & FPS & \#triangles \\
\hline
Instant-NGP &      &     &             \\
Fine-tuned  &      &     &            \\
\bottomrule
\end{tabular}%
\caption{Experiment on transparent dataset}
\label{tab:transparent}
\end{table}

==> fig/comaprison-with-mobile-nerf/item.tex <==
% \begin{figure}
%     \centering
%     \noindent\includegraphics[width=\columnwidth]{fig/transparency-comparison-with-mobilenerf.pdf} 
%     \caption{\textbf{Comparison with MobileNeRF~\cite{chen2022mobilenerf}.} Our approach can represent transparency 
%  whereas MobileNeRF fails.\GS{Update bottle with best results. Also add background texture to Shelly scene.}}\label{fig:comapre-mobilenerf}
% \end{figure}

==> fig/mesh-comparison/item.tex <==
\begin{figure}
    \centering
    \noindent\includegraphics[width=0.8\columnwidth]{fig/mesh-comparisons.pdf} 
    \caption{\textbf{Mesh reconstruction}. Our reconstructed mesh provides a good representation of the underlying object.} \label{fig:mesh-comparisons}
\end{figure}

==> fig/nerf-synthetic/item.tex <==
\begin{figure*}[t!]
    \centering
    \noindent\includegraphics[width=0.9\textwidth]{fig/nerf-synthetic} 
    \caption{\textbf{Visualization of nerf-synthetic dataset.} a) Ground truth, b) instant-ngp with spherical gaussians, c) fine-tuning the meshes produced by our quadrature field (\ref{sec:finetuning}), d) baked neural features using 4096 texture map, and e) using 8192 texture map.
   A larger texture size enables more detailed reconstruction. Notice that our approach is able to represent transparency in the drums.
    }
    \label{fig:nerf-synthetic}
\end{figure*}

==> fig/omega.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\includegraphics[width=.5\linewidth]{fig/effect-omega.pdf}
    \caption{\textbf{Learned quadrature field from \cref{fig:teaser}}. a) quadrature field along a cross-section, b) zero crossings at $\omega=1$ and c) zero crossings at $\omega=50$. \GS{Add a different figure showing number of quadrature points}
    }
    \label{fig:onion}
\end{wrapfigure}

==> fig/splash.tex <==
\begin{figure}[ht]
    \centering
    \noindent\includegraphics[width=0.5\linewidth]{fig/splash.png} 
    \caption{Our approach performs in real-time on variety of devices and is able to represent variety of scenes including transparent objects faithfully. \todo{Fancy figure with RGB, grad field and mesh.}}
    \label{fig:splash}
\end{figure}
